On Optimizing Replica Migration in Distributed Cloud Storage Systems

With the wide adoption of large-scale Internet services and big data, the cloud has become the ideal environment to satisfy the ever-growing storage demand, thanks to its seemingly limitless capacity, high availability and faster access time. In this context, data replication has been touted as the ultimate solution to improve data availability and reduce access time. However, replica placement systems usually need to migrate and create a large number of data replicas over time between and within data centers, incurring a large overhead in terms of network load and availability. In this paper, we propose CRANE, an effiCient Replica migrAtion scheme for distributed cloud Storage systEms. CRANE complements any replica placement algorithm by efficiently managing replica creation in geo-distributed infrastructures by (1) minimizing the time needed to copy the data to the new replica location, (2) avoiding network congestion, and (3) ensuring a minimal availability of the data. Our results show that, compared to swift (the OpenStack project for managing data storage), CRANE is able to minimize up to 30% of the replica creation time and 25% of inter-data center network traffic, while ensuring the minimum required availability of the data.

==> SolutionDesign_2.tex <==
In this section we will describe our heuristic algorithm for the replicas migration problem. Given an initial and a target replicas mapping in data centers, the goal of this algorithm is to find the best sources for copying the replicas and the best sequence to send them. 

%\subsection{Design rationale}
The goal of the proposed algorithm is to find the migration sources and sequences that minimize the total migration time. To this end, the following sights can be used to find an efficient replica creation and migration sequence that: (1) avoids redundancy, (2) selects the source of data and paths having more available bandwidth and (3) avoid idle time between sequences.


Our  heuristic  solution  is  described  in  Algorithm 1.  Given the initial  and target partitions location i.e. $C^I$ and $C^F$ , Algorithm 1 returns a set $Q$ of sequences $Q_{i}$ for migration. Each sequence contains an ordered set of replicas to be migrated on a time period with considering the minimum availability per partition constraint. After each migration of $Q_{i}$ all the cloud storage components will receive this new intermediate partitions placement, so that they will redirect requests to the right partition locations. Each sequence $Q_{i}$ is an ordered sequence containing the replica of each partitions that would be migrated in order to minimize migration time. 

Initially, $P$ contains the set of partitions that need to be created/migrated. This set can be computed based on the initial and the final partition locations (i.e., $C^I$ and $C^F$). We then initialize $Q$ that should contain the sequence of replicas to be migrated. In line 3, we initialize a variable $i$ that denotes the number of the sequence. The core of the algorithm aims to iteratively add a partition replica on ordered sequence $Q_{i}$. We create a new sequence whenever it is not possible anymore to add a replica creation/migration to the current sequence (not possible because otherwise we do not satisfy the minimum replica availability per partition). That is, the variable $available$ define that there still some partitions that can be added to the sequence $Q_i$ . This variable is initialized to $True $ (line 6). 
%
Then, as long as there are some partitions that can be added to the sequence ($available=True$), we iterate over all partitions $P$. And then we choose the replica  $r_b$ from the set of replicas $R_p$ of each partition $p$ that minimizes the migration time. For that we initialize in line 13 a variable $T_{Q_i,R_p,min}$, that represents the minimal migration time of the sequence $Q_{i}$ while including a replica of partition p. We compare in line 15 this variable to $T_{Q_i,r}$ which represents the migration time of the sequence $Q_i$ while including replica $r$. This will allow us to select the best replica $r_b$ of the partition $p$. From those selected replicas, we select the one that minimizes migration time (denoted by $r_s$).  For that, we initialize the variable $T_{Q_i,min}$ that represents the minimal migration time after adding a new replica to the sequence $Q_i$ (line 9). We then choose from all previously selected replicas the replica that  minimizes migration time after adding a new replica (line 20 to 23). The chosen replica is then added to $Q_i$ (line 26). 
The partition $p$ of this replica is then deleted from $P$.

To detect that we cannot add any more replica to the sequence $Q_i$, we iterate over all partition until the variable $available$ becomes $True$. At that time, we add this sequence to $Q$, and start a new sequence as long as we still have partitions in $P$ to migrate/create.

\begin{algorithm}
\caption{Heuristic algorithm for replica migration}
\textbf{require:} Initial configuration $C^I$. \\
\textbf{require:} Final configuration  $C^F$ \\
 \textbf{output:} Sequence for migration \\
\begin{algorithmic}[1]
\STATE $P \leftarrow $ partitions to be migrated
\STATE $Q \leftarrow \{\emptyset\}$
\STATE $i \leftarrow 0$
\WHILE {$P \not=\{\emptyset\} $}
	\STATE $Q_{i} \leftarrow \{\emptyset\}$ 
	\STATE $available \leftarrow True$
	\WHILE {$available == True$}
		\STATE $available \leftarrow False$
		\STATE $T_{Q_i,min} \leftarrow	\infty	$
		\FOR{\textbf{each} $p \in P$}
			\IF{p can be included in $Q_{i}$}
				\STATE $available \leftarrow True$	
				\STATE{ $T_{Q_i,R_p,min} \leftarrow \infty$}
				\FOR{\textbf{each} $r \in R_{p}$}
 					 \IF{$ T_{Q_i, r} < T_{Q_i,R_p,min}$}
    						\STATE $T_{Q_i,R_p,min} = T_{Q_i, r}$
    						\STATE $r_{b}  = r$
   					\ENDIF
 				\ENDFOR
 				\IF{$T_{Q_i,R_p,min} < T_{Q_i,min}$}
 					\STATE $T_{Q_i,min} = T_{Q_i,R_p,min} $
 					\STATE $r_{s}  = r_{b}$
				\ENDIF
			\ENDIF
		\ENDFOR
		\STATE $Q_{i} =  Q_{i} \cup r_{s}$
		\STATE $P = P - \{$partition $p$ of replica $r_{s}\}$
	\ENDWHILE
	\STATE $Q = Q \cup Q_{i} $
	\STATE $i \leftarrow i+1$
\ENDWHILE
\STATE \textbf{return} Q
\label{Algo}
\end{algorithmic}
\end{algorithm}
